The influence of Host Galaxies in Type Ia Supernova Cosmology

We use a sample of 1338 spectroscopically confirmed and photometrically classified Type Ia Supernovae (SNe Ia), sourced from the CSP, CfA, SDSS-II, and SNLS supernova samples, to examine the relationships between SNe Ia and the galaxies that host them. Our results provide confirmation with improved statistical significance that SNe Ia, after standardization, are on average more luminous in massive hosts (significance $\rm > 5 \sigma$), and decline more rapidly in massive hosts (significance $\rm > 9\sigma$) and in hosts with low specific star formation rates (significance $\rm > 8\sigma$). We study the variation of these relationships with redshift and detect no evolution. We split SNe Ia into pairs of subsets that are based on the properties of the hosts, and fit cosmological models to each subset. Including both systematic and statistical uncertainties, we do not find any significant shift in the best-fit cosmological parameters between the subsets. Among different SN Ia subsets, we find that SNe Ia in hosts with high specific star formation rates have the least intrinsic scatter ($\rm \sigma_{int}=0.08\pm0.01$) in luminosity after standardization.

==> comment.tex <==


Do the authors want to comment on the host-less SNe here?
- We have addressed it.


In the pp beginning, "Two more selection steps are required...", I have a question. Photometrically classified SNe Ia tend to be fainter and more distant than those with spectra. If evolution of SNe luminosity occurs with redshift, one might see a systematic behaviour in Fig 1 (which I didn't see). My question regards the removal of the objects that were outside of the specified ellipse: was that removal uniform around the ellipse?

-Yes the rejection was almost uniform. I have a plot to show this. 

Fig 2 and relevant text: Was this photometry measured at a variety of tau?

- Yes.

2.4.1 2nd pp. I see that this work was done in Sato (2014), but I wonder how well it works? Was it tested using SNe and galaxies with spectroscopic redshifts?

-Yes.

2.4.4 The section is unclear as to what kind of data is used in the Z-PEG fitting? Photometry, spectra, both? As the authors note, having UV and IR photometry improves the SFR estimates greatly, so it should be noted specifically what photometry is available. 

- We have used ugriz photomery to fit SEDs. We have now clarified it in the paper.

Fig 5 is particularly troubling because of the striping evident. Most readers will look at this figure and notice the striping, and think that is the principal result. I suggest the authors try a different SP modeling code such as Le Phare (http://www.cfht.hawaii.edu/~arnouts/LEPHARE/lephare.html) which is also based on PEGASE and does not have the strong issues with template-induced striping seen here (I am not one of the originators of Le Phare and have nothing to gain by recommending it). While I don't think that the primary results will change here, I am worried about covariance in the derivations of the total stellar masses

- We have computed host galaxy properties with Le PHARE. The stripings has improved  and the results are unchanged. For example, we compare offsets in stretch in mass subsets from this subsample. Using Z-PEG results, for photometrically classified SNe Ia, we find that the offset in stretch between massive and lower mass hosts is 0.4 with a significance of $\rm 5\sigma$. For the same subsample, using results from Le PHARE, we find the offset to be 0.34 with a significance of  $\rm 4.5\sigma$.}

We have added a section to describe it (Section 4.2). I also attach a plot of Le PHARE. 





Also, not having access to the full table, I can't figure out what fraction of the galaxies are in the non-star forming class. It would seem to me that the result of stretch vs sSFR is strongest between the completely non-star forming galaxies and the rest of the sample. That is, you don't have to divide the entire sample evenly in half. This in itself may be a total stellar mass issue, as the non-star forming galaxies look to have a more massive mean than the rest of the sample.

- 23 % of the sample are non-starforming. We have divided the sample at  median host properties to have almost the same number of SNe Ia in each subset. We agree that the result is strongest when we divide the sample in active and passive hosts. 


Fig 7 and discussion - I'm wondering why a K-S test wasn't also performed.

-We have added a section to present a K-S test (Section 3.4). 

Finally, the principal result here can be thought of as being due to metallicity differences in the hosts, which resulted in different SNe Ia progenitor metallicities. I would have thought the authors would discuss that point in the conclusions, and perhaps mention the possible physical underpinnings of the Phillips relation, even if the words are purely speculative.

- We have added a paragraph in the Summery section on this. 
